The ICL Consistency Test

Just like the previous generation of task-tuned models, large language models (LLMs) that are adapted to tasks via prompt-based methods like in-context-learning (ICL) perform well in some setups but not in others. This lack of consistency in prompt-based learning hints at a lack of robust generalisation. We here introduce the ICL consistency test -- a contribution to the GenBench collaborative benchmark task (CBT) -- which evaluates how consistent a model makes predictions across many different setups while using the same data. The test is based on different established natural language inference tasks. We provide preprocessed data constituting 96 different 'setups' and a metric that estimates model consistency across these setups. The metric is provided on a fine-grained level to understand what properties of a setup render predictions unstable and on an aggregated level to compare overall model consistency. We conduct an empirical analysis of eight state-of-the-art models, and our consistency metric reveals how all tested LLMs lack robust generalisation.

==> text_fragments.tex <==

% DEFINING CONSISTENCY MEASURES IN A FORMAL WAY:
\subsubsection{Consistency}
\label{subsubsec:consistency_templates}
We define the consistency $c_{\pi}$ of a model $\pi$ as the inverse of the entropy of its prediction on the same data point across different setups (e.g. how much a model prediction changes when we use different instructions).
%or internal consistency, showing how consistent one value of an invariance condition is compared to all other values (e.g. how similar are responses to instruction A compare to instructions B, C and D).
We calculate the entropy $\mathcal{H}_{\lambda_{ic}}$ of the predictions $\pi(x_i)$ of a model $\pi$ given an input $x_i$ across different values of $\lambda_{ic}$.
We then sum over all available inputs to get 
\begin{equation*}
c_{\pi} = 1 / \sum_{x_i\in X} \mathcal{H}_{\lambda_{ic}}(\pi(x_i)|x_i; \pi)
\end{equation*}

%We estimate \textbf{internal consistency} by calculating  Cohen's $\kappa$ \citep{cohen1960coefficient}, a measure of interrater reliability.
%Sensitivity to changes in the instructions is a general problem in ICL \citep{mishra2021reframing}.
We apply this metric of consistency across all available P3 instructions for ANLI.
If we compare different models on their external consistency, we find in Figure~\ref{subfig:consistency_templates_per_model} that size and tuning influence a model's consistency across instructions. 

To get a better understanding of the contributions of each individual type of instruction to $c$, we further define the consistency of a condition $c_{\lambda}$ as Cohen's $\kappa$ \citep{cohen1960coefficient}, a measure of interrater reliability, across all possible realizations of $\lambda$.
The metric $c_{\lambda}$ allows us to estimate the agreement of one instruction with all other instructions.
Figure~\ref{subfig:consistency_templates_per_template} shows $\kappa$s for each instruction.
The order of least to most consistent instruction across models is very similar with highly consistent instructions also yielding the best accuracies (see Figure~\ref{subfig:heatmap_performance_templates}).
We can see that the improvement in consistency stems from larger, instruction-tuned models achieving higher consistency across `bad templates.



% FORMALISATIONS FOR LINEAR REGRESSION FOR INTERACTIONS
Lastly, we show interactions between different factors by fitting a linear regression for each possible combination of $\lambda_i$ and $\lambda_j$ while introducing an interaction term $\lambda_i \times \lambda_j$ such that $Acc_{\pi} = \beta_i\lambda_i + \beta_j\lambda_j + \beta_{ij}\lambda_i \times \lambda_j + \beta_0$. 

Figure~\ref{fig:interactions} shows the $\beta_{ij}$ values for conditions that are significantly interacting with each other.
Overall, interaction patterns are similar between the two smaller and the two larger models.
We find most interactions in conditions that are related to the form of instructions of the target example that have been used (such as 'Instructions' or 'Instruction quality').
This is interesting, as we have seen in the main effects that the quality of instructions has the largest influence on accuracy. 
The interaction patterns indicate that instructions are also the most volatile, with their improvements being dependent on the other factors in the setup. 
Interactions of instructions with calibration are especially prominent. 



% THIS IS AN ATTEMPT AT PUTTING CONDITIONS INTO TABLE, RETRY LATER
% CURRENT PROBLEM: WITH THE STANDARD TABLE TEMPLATE FOR EMNLP, I CANNOT EXPAND LIMIT THE TABLE TO LINEWIDTH WITHOUT SHRINKING IT TO TINY PROPORTIONS USING \resizebox{\textwidth}{!}{..} OR CHANGING THE FORMATTING OF THE TABLE USING \begin{tabular}{|p{0.35\linewidth}|p{0.55\linewidth}|}
\begin{table*}[htbp]
\centering

\begin{tabular}{ll}
\hline
\textbf{Variance Condition} & \textbf{Description} \\
\hline
Size & We consider models with 7B, 13B, 30B, and 65B parameters. We create a separate analysis for each model size due to its major influence on predictions and interactions with other conditions. \\
Instruction tuning & Models are either instruction-tuned or not (`vanilla'). \\
Calibration & We calibrate model outputs using content-free prompts following \citet{zhao2021calibrate} or not. \\
n-shots & We use many ($k$ = 5) or few ($k$ = 2) in-context examples in the prompt. \\
Instruction quality & We use semantically equivalent but differently performing instruction templates (high- vs. low-performing). \\
Balanced labels & We ensure that the labels of in-context examples are distributed uniformly or not. \\
\hline
\end{tabular}\\
\begin{tabular}{ll}
\hline
\textbf{Invariance Condition} & \textbf{Description} \\
\hline
Cross-templates & We draw the in-context instructions randomly from all available instruction templates for a specific dataset or use the same instructions as for the target. \\
Cross-task & We use an extractive question-answering task (SQuAD; open-label space), another classification task (QQP; closed-but-incongruent label space), or the same task as the target (ANLI). \\
Instructions & We use different instructions that are similar in quality. \\
\hline
\end{tabular}%

\caption{Variance and Invariance conditions}
\label{tab:conditions}
\end{table*}


\iffalse
\subsubsection{Variance conditions}
\label{subsubsec:v_condtions}
We test 5 binary and 1 quaternary $\lambda_{var}$s.
In the following, we \emph{shortly} describe each of them and provide a detailed description and motivation in Appendix~\ref{app:conditions_details}.

%task: easy [MNLI] vs. hard [ANLI] (binary)
\paragraph{Size\footnote{We expect size to have such a major influence on predictions and interactions with other conditions that we create a separate analysis for each model size.}} We consider models with 7B, 13B, 30B and 65B parameters.

\paragraph{Instruction tuning} Models are either instruction-tuned or not (`vanilla').

\paragraph{Calibration} We calibrate model outputs using \emph{content-free} prompts following \citet{zhao2021calibrate} or not.

\paragraph{n-shots} We use many ($k$ = 5) or few ($k$ = 2) in-context examples in the prompt.

\paragraph{Instruction quality} We use semantically equivalent but very differently performing instruction-templates (high- vs. low-performing; more details in Section~\ref{subsec:probing_templates}).

\paragraph{Balanced labels} We ensure that the labels of in-context examples are distributed uniformly or not.

\subsubsection{Invariance conditions}
\label{subsubsec:i_condtions}
We test 3 binary and 1 ternary $\lambda_{inv}$s.
In the following, we shortly describe each of the tested $\lambda_{inv}$.

\paragraph{Cross-templates} We draw the in-context instructions randomly from all available instruction templates for a specific dataset or use the same instructions as for the target.

\paragraph{Cross-task} We use another classification task (QQP; closed-but-incongruent label space) in-context or the same task as the target task (ANLI).

\paragraph{Instructions} We use different instructions that are similar in quality (more details in Section~\ref{subsec:probing_templates}).

\paragraph{One label} We use only in-context example that have a single randomly selected label or not.
\fi



